Vulpedia: Detecting Vulnerable Ethereum Smart Contracts via Abstracted Vulnerability Signatures

Recent years have seen smart contracts are getting increasingly popular in building trustworthy decentralized applications. Previous research has proposed static and dynamic techniques to detect vulnerabilities in smart contracts. These tools check vulnerable contracts against several predefined rules. However, the emerging new vulnerable types and programming skills to prevent possible vulnerabilities emerging lead to a large number of false positive and false negative reports of tools. To address this, we propose Vulpedia, which mines expressive vulnerability signatures from contracts. Vulpedia is based on the relaxed assumption that the owner of contract is not malicious. Specifically, we extract structural program features from vulnerable and benign contracts as vulnerability signatures, and construct a systematic detection method based on detection rules composed of vulnerability signatures. Compared with the rules defined by state-of-the-arts, our approach can extract more expressive rules to achieve better completeness (i.e., detection recall) and soundness (i.e., precision). We further evaluate Vulpedia with four baselines (i.e., Slither, Securify, SmartCheck and Oyente) on the testing dataset consisting of 17,770 contracts. The experiment results show that Vulpedia achieves best performance of precision on 4 types of vulnerabilities and leading recall on 3 types of vulnerabilities meanwhile exhibiting the great efficiency performance.

==> fig/eval_fn3.tex <==
\begin{figure}[t] 
\vspace{-5mm}
	%\begin{minipage}%[t]{1.0\linewidth}
\begin{lstlisting}
function callTokenFallbackIfNeeded(address sender, address recipient, uint amount, bytes data) internal preventReentrancy {
  uint length;
  // Retrieve the size of code on the recipient address
  assembly {length := extcodesize(recipient) }
  if (length > 0) {
    recipient.call(abi.encodeWithSignature("tokenFallback(address,uint256,bytes)", sender, amount, data));}
}
\end{lstlisting}
\vspace{-2mm}
\caption{\textbf{CB16}: a real case of unchecked low-level-call, which is a TP for \ourTool  but a FN for \smartcheck.}\label{fig:evaluation:fn3}
%	\end{minipage}
\vspace{-2mm}
\end{figure} 


==> fig/eval_fn4.tex <==
\begin{figure}[t] 
\vspace{-2mm}
	%\begin{minipage}%[t]{1.0\linewidth}
\begin{lstlisting}
function updateRate(uint newTokenInWei) public onlyOwner {
  assert(!finalized);
  assert(isUpdatable);
  assert(now <= startsAt);
  CrowdsaleExt lastTierCntrct=CrowdsaleExt(getLastTier());
  assert(!lastTierCntrct.finalized());
  pricingStrategy.updateRate(newTokenInWei);
}
\end{lstlisting}
\vspace{-2mm}
\caption{\textbf{CB17}: a real case of time manipulation, which is a TP for \ourTool  but a FN for \slither and \oyento.}\label{fig:evaluation:fn4}
%	\end{minipage}
\vspace{-1mm}
\end{figure} 


==> fig/eval_fp1.tex <==
\begin{figure}[t]
\begin{minipage}[t]{1.0\linewidth}	
\begin{lstlisting}
contract BancorLender {
  ERC constant public bancorToken =
    ERC(0x1f573d6fb3f13d689ff844b4ce37794d79a7ff1c);
  function closePosition(uint _idx) public {
    ...
    bancorToken.transfer(agets[_idx].lender, amount);
    return;
    } }
	\end{lstlisting}
\end{minipage}
\caption{A real case of using SIG3 (a hard-coded address at line 3), a FP of \emph{reentrancy} for \slither.}
\label{fig:evaluation:fp1}
\end{figure}


==> fig/eval_fp2.tex <==
\begin{figure}[t] 
\vspace{-2mm}
	%\begin{minipage}%[t]{1.0\linewidth}
	\begin{lstlisting}
interface P3D {
	function buy(address _playerAddress) payable external returns(uint256);
}
contract Crop {
	...
	function buy(address _playerAddress) external payable onlyOwner() {
		P3D(0xB3775fB83F7D12A36E0475aBdD1FCA35c091efBe).buy.value(msg.value)(_playerAddress);
	}
...} 
\end{lstlisting}
\vspace{-2mm}
\caption{\textbf{CB5}: a  real case of using DM2,  a FP for \oyento.}\label{fig:evaluation:fp2}
	%	\end{minipage}
	\vspace{-3mm}
\end{figure} 

==> fig/eval_fp3.tex <==
\begin{figure}[t]
%\vspace{-3mm}
	%\begin{minipage}%[t]{1.0\linewidth}
\begin{lstlisting}
contract RegDocuments {
 modifier onlyAdmin() {
  if (msg.sender!= admin && msg.sender!=owner) revert();
  ...;
 }
 constructor() {
  admin = msg.sender;
  owner = 0xc238ff50c09787e7b920f711850dd945a40d3232;
 }
 function regstDocs(bytes32 _storKey) onlyAdmin payable{
  uint _value = Storage.regPrice();
  Storage.regstUser.value(_value)(_storKey);
 }		
}
\end{lstlisting}
\caption{a  real case of using a self-defined modifier (DM3), a FP of \emph{reentrancy} for
	\slither~and~\oyento. }\label{fig:evaluation:fp3}
\end{figure}



==> fig/eval_fp4.tex <==
\begin{figure}[t] 
	%\begin{minipage}%[t]{1.0\linewidth}
\begin{lstlisting}
contract ZethrBankroll is ERC223Receiving {
ZTHInterface public ZTHTKN;
bool internal reEntered;
function receiveDividends() public payable {
  if (!reEntered) {
    ...
    if (ActualBalance > 0.01 ether) {
      reEntered = true;
      ZTHTKN.buyAndSetDivPercentage.value(ActualBalance)(address(0x0), 33, "");
    }
} } }
\end{lstlisting}
\caption{A real case of using SIG4 (an execution lock of \codeff{reEntered}), an FP of \emph{reentrancy} for \slither.}\label{fig:evaluation:fp4}
	%	\end{minipage}
\end{figure}



==> fig/eval_fp7.tex <==
\begin{figure}[t]

 %\begin{minipage}%[t]{1.0\linewidth}
\begin{lstlisting}
function destroyDeed() public {
	require(msg.sender == owner);
	if (owner.send(address(this).balance)) {
		selfdestruct(burn);}
}
\end{lstlisting}
\caption{A real FP of \emph{self-destruct abusing} by \slither,  as \codeff{selfdestruct()} is used under two checks at line  2,4 (SIG10).}
\label{fig:evaluation:fp7} %	\end{minipage}

\end{figure} 

==> fig/motivatingExm2.tex <==
\begin{figure*}[t]
	 \vspace{-3mm}
\centering
%\centering
\begin{subfigure}[Second listing]{0.45\linewidth}
\centering
 \begin{minipage}[t]{1.0\linewidth}
 \begin{lstlisting}
contract Auction {
	address currentLeader;
	uint highestBid;
	function bid() payable {
		require(msg.value > highestBid);
		require(currentLeader.send(highestBid)); // Refund the old leader,
		currentLeader = msg.sender;
		highestBid = msg.value; }
}
\end{lstlisting}
\caption{\textbf{CB1}: an unexpected revert  publicly reported by the blog~\cite{consensys}.}\label{fig:motivating2:original}
\end{minipage}
\end{subfigure}
\qquad\qquad
\begin{subfigure}[A listing]{0.45\linewidth}
\begin{minipage}[t]{1.0\linewidth}
 \begin{lstlisting}
contract AuctionPotato {
  address public hestBidder;
  mapping(address => uint256) public funds;
  ......
  function placeBid() public payable returns (bool success) {
  ...
    funds[hestBidder] = funds[hestBidder].add(bid);
    hestBidder.transfer(funds[hestBidder]);
    hestBidder = msg.sender;
  ...} }

 			\end{lstlisting}
 			\caption{\textbf{CB2}: another unexpected revert from a real-world contract.}\label{fig:motivating2:cloned}
 		\end{minipage}
 	\end{subfigure}
 \vspace{-2mm}
 	\caption{Two \emph{unexpected revert} vulnerabilities with big gaps, which are missed by \slither, \oyento and \securify.}\label{fig:motivating2}
 \vspace{-3mm}
 \end{figure*} 

==> fig/motivatingExm3.tex <==
\begin{figure*}[t]
	 \vspace{-3mm}
\centering
%\centering
\begin{subfigure}[Second listing]{0.45\linewidth}
\centering
 \begin{minipage}[t]{1.0\linewidth}
 \begin{lstlisting}
function doAirDrop(address[] _addr, uint256[] _amount, uint256 _ethAmount) onlyOwner public{
    uint256 count = _address.length;
    for (uint256 i = 0; i < count; i++)
    {
      tokenInstance.transfer(_addr[i],_amount[i]);
      if(this.balance >= _ethAmount)
      {
        require(_addr[i].send(_ethAmount));
      }
    }
}
\end{lstlisting}
\caption{an unexpected revert  publicly reported by \slither.}\label{fig:motivating3:original}
\end{minipage}
\end{subfigure}
\qquad\qquad
\begin{subfigure}[A listing]{0.45\linewidth}
\begin{minipage}[t]{1.0\linewidth}
 \begin{lstlisting}
function _paySceneStarOwners(Scene _scene, uint256 fee) private {
    for (uint i = 0; i < _scene.stars.length; i++) {
        address _pornstarOwner;
        (_pornstarOwner) = pornstarsContract.ownerOf(_scene.stars[i]);

        if(_isGoodAddress(_pornstarOwner)) {
            _pornstarOwner.transfer(fee);
        }
    }
  }
\end{lstlisting}
\caption{another unexpected revert which is missed by \slither.}\label{fig:motivating3:cloned}
\end{minipage}
\end{subfigure}
 \vspace{-2mm}
 	\caption{Two similar \emph{unexpected revert} vulnerabilities. The left code can be detected by \slither while the right one cannot.}\label{fig:motivating3}
 \vspace{-3mm}
 \end{figure*} 

==> fig/reentrancy_example.tex <==
\begin{figure}[t]
%\vspace{-3mm}
	%\begin{minipage}%[t]{1.0\linewidth}
\begin{lstlisting}
function withdraw() {
    require(msg.sender == owner);
    uint256 amount = balances[msg.sender];
    require(msg.sender.call.value(amount)());
    balances[msg.sender] = 0;
}
\end{lstlisting}
\caption{an example of Solidity code with reentrancy vulnerability}
\label{fig:reentrancy_example}
\end{figure}

==> fig/sig-extraction.tex <==

\begin{figure*}[!ht]
\footnotesize
\begin{minipage}[t]{0.33\linewidth} 
\centering      
\begin{lstlisting}  
// Code Block A
function buy(ERC20 _token, address[] _exs, uint[] _indexs, uint256[] _values) public payable 
{
  for (uint i=0; i<_exs.length; i++)
  {
    bytes memory data = new bytes(_indexs[i+1] - _indexs[i]);
    if(_token!=address(0) && i > 0)
    {
      transfer(_token, _values[i]);
    }
    else{
      require(_exs[i].call.value(_values[i])(data), "");
    } } }
\end{lstlisting} 
\end{minipage}
\begin{minipage}[t]{0.33\linewidth} 
    \centering 
    \begin{lstlisting} 
// Code Block B
function buy(ERC20 _token, address[] _exs, uint[] _indexs, uint256[] _values) public payable
{
  for (uint i=0; i<_exs.length; i++)
  {
    bytes memory data = new bytes(_indexs[i+1] - _indexs[i]);
    
    
    
    
    


    require(_exs[i].call.value(_values[i])(data), "");
  }
}
\end{lstlisting} 
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}     
\centering      
\begin{lstlisting}  
// Code Block C
function buy(ERC20 _thToken, address[] _exs, uint[] _idxs, uint256[] _values) public payable
{
  for (uint i=0; i<_exs.length; i++)
  {


    if(_thToken.isSpecialToekn)
    {
      transfer(_token, _values[i]);
    }
    else{
    
      require(_exs[i].call.value(_values[i])(data), "");
    } } }
\end{lstlisting}  
\end{minipage}
\caption{Three similar code blocks of Unexpected Revert that are found in real-world contracts.} 
\label{fig:learningSignature}
\end{figure*}

==> fig/table_RDR.tex <==

\begin{table}[t]
	\centering
    \scriptsize
	\caption{The RDRs are built on the rules of the existing scanners and integrate the  DMs unconsidered by these scanners.}	\label{tab:rdr_dm}
	\small
    \vspace{-2mm}
	\begin{tabular}{|c|c|c|}
		\hline
		\textbf{Vul. Type}  & \textbf{Rule} &  \textbf{DM}  \\
		\hline
		Reentrancy &  \slither & DM1 to DM5 \\
		\hline
		Unexpected Revert & \slither & DM6, DM7 \\
        \hline
        Tx.origin Abusing & \smartcheck & DM8  \\
		\hline
		Unchecked L.L.C & \smartcheck & DM9  \\
		\hline
        Selfdestruct Abusing & \slither & DM10   \\
        \hline
	\end{tabular}

	    %\vspace{-5mm}
\end{table}
\normalsize 

==> tables/dm_stat.tex <==



==> tables/old_detection_evaluation.tex <==
\begin{comment}
\begin{table*}[t]
		\footnotesize
 \centering
 \caption{The number of detected vulnerabilities at contract level and true positive (TP) rate of each scanner.}
 \begin{tabular}{|p{11.625em}|p{5.375em}|p{5.375em}|p{5.675em}|}
  \hline
  Vulnerability (Precision Rate) & \textsc{Slither v.0.4.0} & \textsc{Oyente v0.2.7} & \textsc{SmartCheck v2.0}  \\
  \hline
  Reentrancy & 623 (3.53\%) & 143 (16.78\%) & \quad\quad$\times$  \\
  \hline
  Abuse of Tx Origin & 67 (28.35\%) & \quad\quad$\times$ & 150 (12.66\%) \\
  \hline
  Unchecked Low-Level-Call & \quad\quad$\times$ & \quad\quad$\times$ & 773 (28.71\%) \\
  \hline
  Unexpected Revert & 2678 (8.25\%) & \quad\quad$\times$ & 289 (69.20\%) \\
  \hline
%  Time\newline{}Manipulation & 1387\newline{}(100\%) & \multicolumn{1}{p{3.375em}|}{480\newline{}(100\%)} & \multicolumn{1}{p{3.375em}|}{37\newline{}(100\%)} & 3597\newline{}(100\%) \\
%  \hline
  Self Destruct & 54 (5.56\%) & \quad\quad$\times$ & \quad\quad$\times$  \\
  \hline
 \end{tabular}%
 \label{tab:old_rq1}%
\end{table*}%
\end{comment}

==> tables/signatures <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"ID","cspan":1,"rspan":1,"markup":[1,2]},{"value":"Signatures","cspan":1,"rspan":1,"markup":[1,10]},{"value":"V/B","cspan":1,"rspan":1,"markup":[1,3]},{"value":"Type","cspan":1,"rspan":1,"markup":[1,4]},{"value":"Description","cspan":1,"rspan":1,"markup":[1,11]}],[{"value":"1","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy_call_with_money","cspan":1,"rspan":1,"markup":[1,26]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"reentrancy calls with sending money","cspan":1,"rspan":1,"markup":[1,35]}],[{"value":"2","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy_call_nomoney_send","cspan":1,"rspan":1,"markup":[1,28]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"reentrancy calls without sending money; use send operation","cspan":1,"rspan":1,"markup":[1,58]}],[{"value":"3","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy_call_nomoney\n_transfer","cspan":1,"rspan":1,"markup":[1,33]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"reentrancy calls without sending money; use transfer operation","cspan":1,"rspan":1,"markup":[1,62]}],[{"value":"4","cspan":1,"rspan":1,"markup":[1,1]},{"value":"suicidal_if","cspan":1,"rspan":1,"markup":[1,11]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"selfdestruct","cspan":1,"rspan":1,"markup":[1,12]},{"value":"selfdestruct operation in if statement","cspan":1,"rspan":1,"markup":[1,38]}],[{"value":"5","cspan":1,"rspan":1,"markup":[1,1]},{"value":"suicidal_require","cspan":1,"rspan":1,"markup":[1,16]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"selfdestruct","cspan":1,"rspan":1,"markup":[1,12]},{"value":"selfdestruct operation in require statement","cspan":1,"rspan":1,"markup":[1,43]}],[{"value":"6","cspan":1,"rspan":1,"markup":[1,1]},{"value":"tx_require_assert","cspan":1,"rspan":1,"markup":[1,17]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"tx-origin","cspan":1,"rspan":1,"markup":[1,9]},{"value":"tx.origin operation in require or assert statement, use tx to   compare with addresses","cspan":1,"rspan":1,"markup":[1,86]}],[{"value":"7","cspan":1,"rspan":1,"markup":[1,1]},{"value":"tx_if","cspan":1,"rspan":1,"markup":[1,5]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"tx-origin","cspan":1,"rspan":1,"markup":[1,9]},{"value":"tx.origin operation in if statement, use tx to compare with   addresses","cspan":1,"rspan":1,"markup":[1,71]}],[{"value":"8","cspan":1,"rspan":1,"markup":[1,1]},{"value":"unchecked_LLC_require","cspan":1,"rspan":1,"markup":[1,21]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"unchecked low-level-call in require statements","cspan":1,"rspan":1,"markup":[1,46]}],[{"value":"9","cspan":1,"rspan":1,"markup":[1,1]},{"value":"unchecked_LLC_if","cspan":1,"rspan":1,"markup":[1,16]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"unchecked low-level-call in if statements","cspan":1,"rspan":1,"markup":[1,41]}],[{"value":"10","cspan":1,"rspan":1,"markup":[1,2]},{"value":"unchecked_LLC_return","cspan":1,"rspan":1,"markup":[1,20]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"unchecked low-level-call with return statement","cspan":1,"rspan":1,"markup":[1,46]}],[{"value":"11","cspan":1,"rspan":1,"markup":[1,2]},{"value":"unchecked_LLC_assign","cspan":1,"rspan":1,"markup":[1,20]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"assign unchecked low-level-call return value to variable","cspan":1,"rspan":1,"markup":[1,56]}],[{"value":"12","cspan":1,"rspan":1,"markup":[1,2]},{"value":"unchecked_send_require","cspan":1,"rspan":1,"markup":[1,22]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"unchecked send operation in require statement","cspan":1,"rspan":1,"markup":[1,45]}],[{"value":"13","cspan":1,"rspan":1,"markup":[1,2]},{"value":"unchecked_send_if","cspan":1,"rspan":1,"markup":[1,17]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"unchecked send operation in if statement","cspan":1,"rspan":1,"markup":[1,40]}],[{"value":"14","cspan":1,"rspan":1,"markup":[1,2]},{"value":"unchecked_send_return","cspan":1,"rspan":1,"markup":[1,21]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"unchecked send with return statement","cspan":1,"rspan":1,"markup":[1,36]}],[{"value":"15","cspan":1,"rspan":1,"markup":[1,2]},{"value":"unchecked_send_assign","cspan":1,"rspan":1,"markup":[1,21]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"assign unchecked send return value to variable","cspan":1,"rspan":1,"markup":[1,46]}],[{"value":"16","cspan":1,"rspan":1,"markup":[1,2]},{"value":"revert_send_in_for","cspan":1,"rspan":1,"markup":[1,18]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"unexpected revert","cspan":1,"rspan":1,"markup":[1,17]},{"value":"send operation in for loop","cspan":1,"rspan":1,"markup":[1,26]}],[{"value":"17","cspan":1,"rspan":1,"markup":[1,2]},{"value":"revert_transfer_in_for","cspan":1,"rspan":1,"markup":[1,22]},{"value":"T","cspan":1,"rspan":1,"markup":[1,1]},{"value":"unexpected revert","cspan":1,"rspan":1,"markup":[1,17]},{"value":"transfer operation in for loop","cspan":1,"rspan":1,"markup":[1,30]}],[{"value":"18","cspan":1,"rspan":1,"markup":[1,2]},{"value":"reentrancy_identity_check","cspan":1,"rspan":1,"markup":[1,25]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"Check identity of access before transaction.","cspan":1,"rspan":1,"markup":[1,44]}],[{"value":"19","cspan":1,"rspan":1,"markup":[1,2]},{"value":"reentrancy_transfer_to_fixed\n_address","cspan":1,"rspan":1,"markup":[1,37]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"The transfer addresses is previously initialized with a   hard-coded addresses","cspan":1,"rspan":1,"markup":[1,78]}],[{"value":"20","cspan":1,"rspan":1,"markup":[1,2]},{"value":"reentrancy_selfdefined_modifier","cspan":1,"rspan":1,"markup":[1,31]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"Use self-defined modifier to protect function from malicious   access","cspan":1,"rspan":1,"markup":[1,69]}],[{"value":"21","cspan":1,"rspan":1,"markup":[1,2]},{"value":"reentrancy_execution_lock","cspan":1,"rspan":1,"markup":[1,25]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"Leverage execution locks to limit reentrancy","cspan":1,"rspan":1,"markup":[1,44]}],[{"value":"22","cspan":1,"rspan":1,"markup":[1,2]},{"value":"reentrancy_update_balance\n_before_transfer","cspan":1,"rspan":1,"markup":[1,42]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"reentrancy","cspan":1,"rspan":1,"markup":[1,10]},{"value":"Update balance before conducting a payment","cspan":1,"rspan":1,"markup":[1,42]}],[{"value":"23","cspan":1,"rspan":1,"markup":[1,2]},{"value":"revert_no_require_statement","cspan":1,"rspan":1,"markup":[1,27]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"unexpected revert","cspan":1,"rspan":1,"markup":[1,17]},{"value":"No require for transfer operation to avoid unexpected revert","cspan":1,"rspan":1,"markup":[1,60]}],[{"value":"24","cspan":1,"rspan":1,"markup":[1,2]},{"value":"revert_transfer_to_same_address","cspan":1,"rspan":1,"markup":[1,31]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"unexpected revert","cspan":1,"rspan":1,"markup":[1,17]},{"value":"Transfer to the same address in loop","cspan":1,"rspan":1,"markup":[1,36]}],[{"value":"25","cspan":1,"rspan":1,"markup":[1,2]},{"value":"tx_compare_with_msgsender","cspan":1,"rspan":1,"markup":[1,25]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"tx-origin","cspan":1,"rspan":1,"markup":[1,9]},{"value":"Compare tx.origin with msg.sender","cspan":1,"rspan":1,"markup":[1,33]}],[{"value":"26","cspan":1,"rspan":1,"markup":[1,2]},{"value":"uncheckedLLC_checked","cspan":1,"rspan":1,"markup":[1,20]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"low level call","cspan":1,"rspan":1,"markup":[1,14]},{"value":"Check low-level-calls","cspan":1,"rspan":1,"markup":[1,21]}],[{"value":"27","cspan":1,"rspan":1,"markup":[1,2]},{"value":"suicidal_strict_identity_check","cspan":1,"rspan":1,"markup":[1,30]},{"value":"F","cspan":1,"rspan":1,"markup":[1,1]},{"value":"selfdestruct","cspan":1,"rspan":1,"markup":[1,12]},{"value":"Add strict identity check before selfdestruct operation","cspan":1,"rspan":1,"markup":[1,55]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}}]},"options":{"table_caption":"","table_label":"tab:my-table"}}

==> tables/signatures.tex <==
\begin{comment}
\scriptsize
\begin{table*}[h]
	\centering
	\caption{Summarized Signatures.}
	\begin{tabular}{|p{6mm}|p{60mm}|p{23mm}|p{16mm}|p{40mm}|}
    \hline
    Index & Name & Vulnerable/Benign & Vulnerability& Description \\
    \hline
    1 & reentrancy\_external\_call\_with\_money & v & reentrancy & reentrancy calls with sending money \\
    \hline
    2 & reentrancy\_external\_call\_no\_money\_send & v & reentrancy & reentrancy calls without sending money; use send operation \\
    \hline
    3 & reentrancy\_external\_call\_no\_money\_transfer & v & reentrancy & reentrancy calls without sending money; use transfer operation \\
    \hline
    4 & selfdestruct\_if & v & suicidal & selfdestruct operation in if statement \\
    \hline
    5 & selfdestruct\_require & v & suicidal & selfdestruct operation in require statement \\
    \hline
    6 & frontrunning\_tx\_require & v & tx-origin & tx.origin operation in require or assert statement; use tx to compare with addresses \\
    \hline
    7 & frontrunning\_tx\_if & v & tx-origin & tx.origin operation in if statement; use tx to compare with addresses \\
    \hline
    8 & unchecked\_low-level-call\_require & v & low-level-call & unchecked low-level-call in require statements \\
    \hline
    9 & unchecked\_low-level-call\_if & v & low-level-call & unchecked low-level-call in if statements \\
    \hline
    10 & unchecked\_low-level-call\_return & v & low-level-call &  \\
    \hline
    11 & unchecked\_low-level-call\_assign & v & low-level-call &  \\
    \hline
    12 & unchecked\_send\_require & v & low-level-call & unchecked send operation in require statement \\
    \hline
    13 & unchecked\_send\_if & v & low-level-call & unchecked send operation in if statement \\
    \hline
    14 & unchecked\_send\_return & v & low-level-call & \\
    \hline
    15 & unchecked\_send\_assign & v & low-level-call &  \\
    \hline
    16 & dos\_for\_send & v & unexpected revert & \\
    \hline
    17 & dos\_for\_transfer & v & unexpected revert & \\
    \hline
    18 & access\_control\_by\_identity\_check & b & reentrancy & Check identity of access before transaction. \\
    \hline
    19 & hard\_coding\_address\_of\_payee & b & reentrancy & The transfer addresses is previously initialized with a hard-coded addresses. \\
    \hline
    20 & use\_self-defined\_modifier & b & reentrancy & Use self-defined modifier to protect function from malicious access. \\
    \hline
    21 & execution\_locks & b & reentrancy & Leverage execution locks to limit reentrancy. \\
    \hline
    22 & update\_balance\_before\_payment & b & reentrancy & Update balance before conducting a payment. \\
    \hline
    23 & no\_require\_for\_transfer & b & unexpected revert & No require for transfer operation to avoid unexpected revert. \\
    \hline
    24 & transfer\_to\_same\_address & b & unexpected revert & Transfer to the same address in loop. \\
    \hline
    25 & compare\_tx\_with\_sender & b & tx-origin & Compare tx.origin with msg.sender. \\
    \hline
    26 & check\_low-level-call & b & low-level-call & Check low-level-calls. \\
    \hline
    27 & identity\_check\_before\_suicidal & b & suicidal & Add strict identity check before selfdestruct operation. \\
    \hline
	\end{tabular}
\label{tab:signatures}
\end{table*} 
\end{comment}
